Backtracking linesearch for conditional gradient sliding

We present a modification of the conditional gradient sliding (CGS) method that was originally developed in \cite{lan2016conditional}. While the CGS method is a theoretical breakthrough in the theory of projection-free first-order methods since it is the first that reaches the theoretical performance limit, in implementation it requires the knowledge of the Lipschitz constant of the gradient of the objective function $L$ and the number of total gradient evaluations $N$. Such requirements imposes difficulties in the actual implementation, not only because that it can be difficult to choose proper values of $L$ and $N$ that satisfies the conditions for convergence, but also since conservative choices of $L$ and $N$ can deteriorate the practical numerical performance of the CGS method. Our proposed method, called the conditional gradient sliding method with linesearch (CGS-ls), does not require the knowledge of either $L$ and $N$, and is able to terminate early before the theoretically required number of iterations. While more practical in numerical implementation, the theoretical performance of our proposed CGS-ls method is still as good as that of the CGS method. We present numerical experiments to show the efficiency of our proposed method in practice.

==> ChapterTwo.tex <==
\chapter{CGS With Line Search}


In Chapter 1 we introduced the CGS algorithm (see Algorithm \ref{Alg:CGS}) and also mentioned the complexity and convergence results under different parameter set up. In the $k^{th}$ outer iteration ($k^{th}$ gradient evaluation) of CGS the parameters $\beta_k$ and $\eta_k$ depend on other constants such as the Lipschitz constant $L$, the diameter $D_{\mathcal{X}}$ of the feasible set $\mathcal{X}$ and also the maximum number of outer iteration $N$. Although in theory these constants do not change the convergence rate of the algorithm with proper setting up of parameters, in practice we might have issue in finding these constants. For example, for large $\mathcal{X}$  finding the the Lipschitz constant $L$ might be expensive in terms of computing and CPU-time consuming. This is a draw back of CGS in practice.

One of the most common methods in optimization  is the back tracking line search \cite{armijo1966minimization}. Line search involves starting with an estimate of the corresponding constant and continue the iterations of the algorithm while some conditions are satisfied. This guessed value of constant will be increased iteratively if the specific condition is violated. 

In this chapter we utilize the line search approach for the Lipschitz constant $L$. Algorithm \ref{Alg:CGSLS} is the generic procedure of CGS with line search (CGS-ls). It starts with a first guess of $L$, that is $L_0$ in the algorithm and while the condition \eqref{Alg:CGSLS:approx} is satisfied the algorithm iterates with the same value of $L_k$ at iteration $k$; once \eqref{Alg:CGSLS:approx} is violated this value will be increased by a multiple of 2 until the condition holds.
%In this Chapter we incorporate the backtracking line search to the conditional gradient sliding method. 
%
%\begin{table}
%	\begin{center}
%		\begin{tabular}{rccc}
%			& Nesterov's & Frank-Wolfe & CGS\\
%			\hline
%			Subproblem & $\Pi_X(\cdot)$ & $\color{red}\min_{x\in X}\langle\cdot, x\rangle$ & {\color{red}$\min_{x\in X}\langle\cdot, x\rangle$}\\
%			{\# subproblem} & $\color{red}\sqrt{{LD_X^2}/{\varepsilon}}$ & ${{L^*(D_X^*)^2}/{\varepsilon}}$ & {${{LD_X^2}/{\varepsilon}}$}\\
%			{\# gradient} & $\color{red}\sqrt{{LD_X^2}/{\varepsilon}}$ & ${{L^*(D_X^*)^2}/{\varepsilon}}$ & {\color{red}$\sqrt{{LD_X^2/\varepsilon}}$}\\
%			\hline
%		\end{tabular}
%		\caption{\label{tab:comparison}Comparing the complexity of algorithms Nesterov's, CG and  CGS}
%	\end{center}
%\end{table}
%\end{comment}

\begin{algorithm}[H]
	\caption{\label{Alg:CGSLS} A CGS-ls algorithm}
	\begin{algorithmic}
		\State Initial point $y_0\in \mathcal{X}$. Set $x_0=y_0$.
		\For {$k=1,2,\ldots$}\\
		Find $L\k >0$ such that \vspace{-.5cm}
		\begin{align}
		\label{Alg:CGSLS:approx}
		f(y\k) \le f(z\k) + \ang{f'(z\k), y\k - z\k} + \frac{L\k}{2}\norm{y\k - z\k}^2 +\frac{\epsilon}{2}\g\k
		\end{align}
		\vspace{-.5cm}
		where 
		\begin{align}
		\label{Alg:CGSLS:gamma}
		\gamma\k = \left\{\begin{array}{ll}
		    1 & k=1 \\
		    \text{Positive solution to } \G\k = \G\km(1-\g\k)& k\ge 2
		\end{array} \right.
		\end{align}
		where $\G\k$ depends on $L\k$ and $\g\k$.
		\begin{align}
		&\hspace{1.5cm}		z\k = (1-\g\k)y\km - \g\k x\km\label{Alg:CGSLS:zk}\\
		&\hspace{1.5cm}		x\k \approx \argmin_{x\in \mathcal{X}}\ang{f'(z\k),x}+\frac{\beta\k}{2}\norm{x-x\km}^2 \label{Alg:CGSLS:xk}\\
		&\hspace{1.5cm}		y\k = (1-\g\k)y\km +\g\k x\k\label{Alg:CGSLS:y}
		\end{align}
%		where the approximation in \eqref{Alg:CGSLS:xk} is in the sense that \vspace{-.3cm}
%		\begin{align}
%		\label{Alg:CGSLS:approx}
%		\ang{\gf (z\k),x\k-x}\le \frac{\beta\k}{2}\pr{\norm{x-x\km}^2-\norm{x\k-x\km}^2-\norm{x-x\k}^2}+\eta\k.
%		\end{align}
		Set\vspace{-.3cm}
		\begin{align}
		\label{Alg:CGSLS:ell}
		\ell\k(x):=\G\k\sum_{i=1}^{k}\frac{\g_i}{\G_i}\br{f(y_i)+\ang{f(z_i),x-z_i}}.
		\end{align}
		\vspace{-.3cm}
		Stop if
		\begin{align}
		\label{Alg:CGSLS:minep}
		f(y\k) - \min_{x\in \X}\ell\k(x)\le \epsilon,
		\end{align}
		\vspace{-.3cm}
		or equivalently,
		\begin{align}
		\label{Alg:CGSLS:maxep}
		\max_{x\in \X}f(y\k)-\ell\k(x)\le \epsilon.
		\end{align}
		\EndFor\\
		Output $y_N$.
	\end{algorithmic}
\end{algorithm}


Note that the approximate solution to $x_k$ in \eqref{Alg:CGSLS:xk}, the approximate solution to the projection problem, is given by the same inner iterations as CGS Algorithm \ref{Alg:CGS} inner iterations depending on parameters $\{\beta_k\}$ and $\{\eta_k\}$. Namely, $x\k = \text{CndG}(f'(z\k),x_{k-1},\beta_k,\eta_k)$. Indeed, if we consider the optimality condition 
\begin{align*}
\ang{\gf (z\k)+\beta\k(x\k-x\km),x\k - x} \le \eta\k,
\end{align*}
for $\eta\k = 0$ we have the exact solution to the projection subproblem which leads to the Nesterov's AG method and for $\eta\k > 0,\ x\k$ is solved with accuracy  $\eta\k$. Also, the $L\k$ in Algorithm \ref{Alg:CGSLS} can be the Lipschitz constant or any other amount that \eqref{Alg:CGSLS:approx} hold. In addition, we can observe that the above method is conceptual only since we have not yet specified the parameters $\{\beta_k\}$, $\{\gamma_k\}$ and $\eta_k$ that are used in the algorithm. Before setting these parameters we first establish some convergence properties for the Algorithm \ref{Alg:CGSLS}.

We begin the proof of the convergence of the above algorithm by first showing some technical results that will be used in the analysis of the Algorithm \ref{Alg:CGSLS}.

\begin{lemma}\label{CGSLS:lem:sumone}
For a given $k$ we have 
\begin{align}\label{CGSLS:lem:sumone:eq}
\G\k\sum_{i=1}^{k}\frac{\g_i}{\G_i}=1.
\end{align}
\end{lemma}
\begin{proof}
Let $1\le i \le k$ then by \eqref{Alg:CGSLS:gamma} we have
\begin{align*}
\frac{1}{\Gamma_i} &= \frac{1-\gamma_i}{\Gamma_i} + \frac{\gamma_i}{\Gamma_i}\\
&= \frac{1}{\Gamma_{i-1}} + \frac{\gamma_i}{\Gamma_i}.
\end{align*}
Now summing up both sides of above inequality for $i=2,\cdots, k$ we get
\begin{align*}
\sum_{i=2}^{k} \frac{1}{\Gamma_{i}}-\frac{1}{\Gamma_{i-1}} = \sum_{i=2}^{k}  \frac{\gamma_i}{\Gamma_i}.
\end{align*}
Hence,
\begin{align*}
\frac{1}{\Gamma_{k}}-1 = \sum_{i=2}^{k}  \frac{\gamma_i}{\Gamma_i}.
\end{align*}
This and also the fact that $\gamma_1=1$ imply the \eqref{CGSLS:lem:sumone:eq}.

\end{proof}


\begin{lemma}\label{CGSLS:lem:epsilonGap}
If \eqref{Alg:CGSLS:minep} or \eqref{Alg:CGSLS:maxep} hold, then 
\begin{align*}
f(y\k)-f^*\le \epsilon.
\end{align*}
\end{lemma}
\begin{proof}
From the definition of $\ell_k(x)$ in \eqref{Alg:CGSLS:ell}, Lemma \ref{CGSLS:lem:sumone} and also the convexity of $f$ for any $x\in \mathcal{X}$ we have
\begin{align*}
\ell\k(x)&=\G\k\sum_{i=1}^{k}\frac{\g_i}{\G_i}\br{f(y_i)+\ang{f(z_i),x-z_i}}\\
&\le \G\k\sum_{i=1}^{k}\frac{\g_i}{\G_i}f(x)\\
&= f(x).
\end{align*}
This implies that $\min_{x\in \mathcal{X}}\ell_k(x)\le f^*$ and therefore,
\begin{align*}
f(y_k) - f^* \le f(y_k) -\min_{x\in \mathcal{X}}\ell_k(x)\le \epsilon.
\end{align*}

\end{proof}


Theorem \ref{CGSLS:mainthm} below describes the main convergence property of the Algorithm \ref{Alg:CGSLS}. 


\begin{theorem}
\label{CGSLS:mainthm}
In Algorithm \ref{Alg:CGSLS} if $\beta\k\ge L\k\g\k$, then
\begin{align*}
f(y\k) - \ell\k(x) &\le \frac{\epsilon}{2} + \G\k\sum_{i=1}^{k}\frac{\g_i\beta_i}{2\G_i}\pr{\norm{x-x_{i-1}}^2 - \norm{x-x)i}^2}\\
&\qquad +\G\k\sum_{i=1}^{k}\frac{\g_i\eta_i}{\G_i} - \sum_{i=1}^{k}\frac{\g_i}{2\G_i}\pr{\beta_i-L_i\g_i}\norm{x_i-x_{i-1}}^2.
\end{align*}
\end{theorem}

\begin{proof}
We have
\begin{align*}
\frac{\ell\k(x)}{\G\k} &\stackrel{\eqref{Alg:CGSLS:ell}}{=} \sum_{i=1}^{k}\frac{\g_i}{\G_i}\br{f(z_i)+\ang{\gf (z_i),x-x_i}+\ang{\gf (z\i),x\i-z\i}}\\
&= \sum_{i=1}^{k}\frac{1}{\G\i}\br{\g\i f(z\i)+\g\i\ang{\gf (z_i),x-x_i} + \ang{\gf (z\i),\g\i(x\i-z\i) }}.
\end{align*}
Here
\begin{align*}
\g\i(x\i-z\i) &\stackrel{\eqref{Alg:CGSLS:y}}{=} y\i-(1-\g\i)y\im - \g\i z\i\\
&\hspace{.15cm} = (y\i-z\i) - (1-\g\i)(y\im - z\i).
\end{align*}
So,
\begin{align*}
\frac{\ell\k(x)}{\G\k} &= \sum_{i=1}^{k}\frac{1}{\G\i}[\g\i f(z\i)+ \ang{\gf (z_i),y\i-z\i} \\
&\qquad - (1-\g\i)\pr{f(z\i)+ \ang{\gf (z\i),y\im - z\i }}+\g\i\ang{\gf (z\i),x-x\i}].
\end{align*}
Note that from \eqref{Alg:CGSLS:zk} and \eqref{Alg:CGSLS:y} we have $y\i-z\i = \g\i(x\i-x\im)$ and 
\begin{align*}
f(z\i)+\ang{\gf (z\i),y\i-z\i} &\ge f(y\i)-\frac{L\i}{2}\norm{y\i-z\i}^2 - \frac{\epsilon}{2}\g\i.
\end{align*}
Also, from convexity of $f$ we have
\begin{align*}
-\pr{f(z\i)+\ang{\gf (z\i),y\im-z\i}}\ge -f(y\im),
\end{align*}
and from \eqref{Alg:CGSLS:approx} we have 
\begin{align*}
\g\i\ang{\gf (z\i),x-x\i}\ge -\frac{\g\i\beta\i}{2}\pr{\norm{x-x\im}^2 - \norm{x\i-x\im}^2 - \norm{x-x\i}^2}-\g\i\eta\i.
\end{align*}
Therefore,
\begin{align*}
\frac{\ell\k(x)}{\G\k}&\ge \sum_{i=1}^{k}\frac{1}{\G\i}\left[f(y\i) - \frac{L\i\g\i^2}{2}\norm{x\i-x\im}^2 - \frac{\epsilon}{2}\g\i-(1-\g\i)f(y\im)\right.\\
&\hspace{1.7cm} \left. -\frac{\g\i\beta\i}{2}\pr{\norm{x-x\im}^2 - \norm{x\i-x\im}^2 - \norm{x-x\i}^2} - \g\i\eta\i\right]\\
&= \sum_{i=1}^{k}\frac{1}{\G\i}f(y\i) - \frac{1-\g\i}{\G\i}f(y\im) - \sum_{i=1}^{k}\frac{\g\i\beta\i}{2\G\i}\pr{\norm{x-x\im}^2 - \norm{x-x\i}^2}\\
&\qquad - \frac{\epsilon}{2}\sum_{i=1}^{k}\frac{\g\i}{\G\i} - \sum_{i=1}^{k}\frac{\g\i}{2\G\i}(L\i\g\i-\beta\i)\norm{x\i-x\im}^2 - \sum_{i=1}^{k}\frac{\g\i\eta\i}{\G\i}.
\end{align*}
Noting that 
\begin{align*}
\sum_{i=1}^{k}\frac{1}{\G\i}f(y\i)-\frac{1-\g\i}{\G\i}f(y\im) \stackrel{\eqref{Alg:CGSLS:gamma}}{=}\frac{f(y\k)}{\G\k},
\end{align*}
and also using Lemma \ref{CGSLS:lem:sumone} we have
\begin{align*}
\frac{\ell\k(x)}{\G\k}&\ge \frac{f(y\k)}{\G\k} - \sum_{i=1}^{k}\frac{\g\beta\i}{2\G\i}\pr{\norm{x-x\im}^2-\norm{x-x\i}^2}\\
&\qquad - \frac{\epsilon}{2\G\k} - \sum_{i=1}^{k}\frac{\g\i}{2\G\i}(L\i\g\i-\beta\i)\norm{x\i-x\im}^2 - \sum_{i=1}^{k}\frac{\g\i\eta\i}{\G\i},
\end{align*}
which implies that
\begin{align*}
f(y\k) - \ell\k(x) &\le \frac{\epsilon}{2} + \G\k\sum_{\g_i\beta_i}^{2\G_i}\pr{\norm{x-x_{i-1}}^2 - \norm{x-x)i}^2}\\
&\qquad +\G\k\sum_{i=1}^{k}\frac{\g_i\eta_i}{\G_i} - \sum_{i=1}^{k}\frac{\g_i}{2\G_i}\pr{\beta_i-L_i\g_i}\norm{x_i-x_{i-1}}^2.
\end{align*}
\end{proof}


As we can see in Theorem \ref{CGSLS:mainthm} and the Algorithm \ref{Alg:CGSLS} the parameters $\{\beta_k\}, \{\gamma_k\}$ and $\{\eta_k\}$ are needed to be specified in a proper way to have the desired convergence result. Clearly, there are many options to choose these parameters to guarantee the convergence of CGS-ls. In our next step we and in corollaries \ref{CGSLS:cor:parSetUp1} and \ref{CGSLS:cor:parSetUp2} we provide two different parameter settings for $\{\beta_k\}, \{\gamma_k\}$ and $\{\eta_k\}$ which lead to optimal complexity bounds on total number of gradient evaluations and also the total number of calls to the linear optimizations oracle.


\begin{corollary}\label{CGSLS:cor:parSetUp1}
If we set 
\begin{align*}
  \beta\k = \frac{2L\k}{k},\quad \g\k = \frac{2}{k+1},\quad \G\k = \frac{2}{k(k+1)},\quad \eta\k = \frac{2L\k\dx}{Nk},
\end{align*}
where $N$ is the max number of iteration and is bounded by
\begin{align*}
    N\ge \sqrt{\frac{2M\dx}{\epsilon}},
\end{align*}
where $M$ is the true value of Lipschitz constant, then for all $x\in \mathcal{X}$
\begin{align*}
    f(y\k)-\ell\k(x)\le \frac{\epsilon}{2}+3\G\k M\dx.
\end{align*}
In particular, the total number of $\gf (\cdot)$ evaluations and linear objective optimization computations are bounded by 
\begin{align*}
    \sqrt{\frac{12M\dx}{\epsilon}}\quad \text{and} \quad \pr{\frac{72M\dx}{\epsilon}+\sqrt{\frac{12M\dx}{\epsilon}}},
\end{align*}
respectively.
\end{corollary}
\begin{proof}
Applying the parameter setting to Theorem \ref{CGSLS:mainthm} we have 
\begin{align*}
    f(y\k) - \ell\k(x)&\le \frac{\epsilon}{2}+\G\k\pr{M\dx + 2M\dx} \\
    &= \frac{\epsilon}{2} + 3\G\k M\dx.
\end{align*}
In particular, \eqref{Alg:CGSLS:minep} is satisfied if 
\begin{align*}
    3\G\k M\dx\le \frac{\epsilon}{2},
\end{align*}
i.e.
\begin{align*}
    \frac{6M\dx}{k(k+1)}\le\frac{\epsilon}{2}, \quad \text{or}\quad k\ge \sqrt{\frac{12M\dx}{\epsilon}}.
\end{align*}
Now by Proposition \ref{CGS:thm:convergence} part (c),
\begin{align*}
    \sum_{k=1}^{N}T\k &\le \sum_{k=1}^{N}\frac{6\beta\k\dx}{\eta\k}+1\\
    &= 6N^2 + N\\
    &\le \frac{72M\dx}{\epsilon}+\sqrt{\frac{12M\dx}{\epsilon}}.
\end{align*}
\end{proof}










\begin{corollary}\label{CGSLS:cor:parSetUp2}
As we set of the parameters in the Algorithm \ref{Alg:CGSLS} as 
\begin{align}
\label{CGSLS:thm:par}
\b\k=L\k\g\k,\quad \G\k=L\k\g\k^2\quad \text{and}\quad \eta\k=\frac{L\k\g\k\dx}{N},
\end{align}
where $N$ is the number of outer iterations, we have,
\begin{align}
f(y\k)-f^*\le \frac{12L}{(k-1)^2}\dx.
\end{align}
In other words, the number of gradient evaluations in Algorithm \ref{Alg:CGSLS} is bounded by
\begin{align}
\OC\pr{\sqrt{\frac{L\dx}{\epsilon}}}.
\end{align}
In addition, the number of LP evaluations in the Algorithm \ref{Alg:CGSLS} is bounded by
\begin{align}
\OC\pr{\frac{L\dx}{\epsilon}}.
\end{align}
\end{corollary}
\begin{proof}
Clearly, with parameter set up in \eqref{CGSLS:thm:par} all conditions \eqref{CGS:thm:ass} of Theorem \ref{CGS:thm:convergence} are satisfied and from part (a) of this theorem with $K$ the total number of iterations we have
\begin{align}\label{CGSLS:thm:a}
    \begin{aligned}
    f(y\k)-f^* &\le \frac{\beta_k\gamma_k}{2}\dx + \G\k\sum_{i=1}^{k}\frac{\eta_i\g_i}{\G_i}\\
    &\le \frac{L\k\g\k^2\dx}{2}+L\k\g\k^2\sum_{i=1}^{k}\frac{L_i\g_i^2\dx}{KL_i\g_i^2}\\
    &=\frac{1}{2}L\k\g\k^2\dx + l\k\g\k^2\dx\\
    &=\frac{3}{2}\G\k \dx.
    \end{aligned}
\end{align}
But for $k>1$ we have $\G\k=\G\km (1-\g\k)$. This implies that 
\begin{align*}
    \frac{1}{\G\km} = \frac{1}{\G\k}-\frac{\g\k}{\G\k}\qquad \forall k>1.
\end{align*}
Therefore,
\begin{align*}
    \sqrt{\frac{1}{\G\k}}-\sqrt{\frac{1}{\G\km}} = \frac{\frac{1}{\G\k}-\frac{1}{\G\km}}{\sqrt{\frac{1}{\G\k}}+\sqrt{\frac{1}{\G\km}}}=\frac{\frac{\g\k}{\G\k}}{\sqrt{\frac{1}{\G\k}}+\sqrt{\frac{1}{\G\km}}}.
\end{align*}
Note that $\G\k = (1-\g\k)\G\km\le\G\km$ and $\G\k=L\k\g\k^2$. Hence,
\begin{align*}
    \sqrt{\frac{1}{\G\k}}-\sqrt{\frac{1}{\G\km}} \ge \frac{\frac{\g\k}{\G\k}}{\sqrt{\frac{1}{\G\k}}+\sqrt{\frac{1}{\G\k}}} = \frac{\g\k}{2\sqrt{\G\k}}=\frac{1}{2\sqrt{L\k}}\ge\frac{1}{2\sqrt{2}L}.
\end{align*}
So performing inductively we get
\begin{align*}
    \sqrt{\frac{1}{\G\k}}-\sqrt{\frac{1}{\G\km}} \ge \frac{k-1}{2\sqrt{2}L},
\end{align*}
then 
\begin{align*}
    \sqrt{\frac{1}{\G\k}} \ge \frac{k-1}{2\sqrt{2}L},
\end{align*}
which implies that 
\begin{align*}
    \G\k \le \frac{8L}{(k-1)^2}.
\end{align*}
Therefore, from \eqref{CGSLS:thm:a} we have
\begin{align}
\label{CGSLS:thm:fbnd}
    \begin{aligned}
    f(y\k)-f^* &\le \frac{3}{2}\cdot \frac{8L}{(k-1)^2}\cdot \dx\\
    & = \frac{12L}{(k-1)^2}\dx.
    \end{aligned}
\end{align}
Also, from part (c) of Theorem \ref{CGS:thm:convergence} and definition of $\eta\k$ we have 
\begin{align}
\label{CGSLS:thm:iter}
\begin{aligned}
    \sum_{k=1}^{N}T\k & = \sum_{k=1}^{N}\frac{6\b\k\dx}{\eta\k}\\
    & = \sum_{k=1}^{N}\frac{6 N L\k\g\k\dx}{L\k\g\k\dx}\\
    & = 6 N^2.
    \end{aligned}
\end{align}
Therefore from \eqref{CGSLS:thm:fbnd} and \eqref{CGSLS:thm:iter} w get that the total number of iterations it takes for the CGS algorithm with line search to get an $\epsilon$-certificate is bounded by $\OC\pr{\sqrt{\nicefrac{L\dx}{\epsilon}}}$ and the number of linear programming evaluations is bounded by $\OC\pr{\nicefrac{L\dx}{\epsilon}}$.
\end{proof}

An observation that we can have from corollaries \ref{CGSLS:cor:parSetUp1} and \ref{CGSLS:cor:parSetUp2} is that in both type of settings of parameter we require the knowledge of $N$, the maximum number of outer iterations or the total number of gradient evaluations. However, we can improve the bound on number of calls to linear optimization oracle or the number of inner iterations in terms of its dependence on $N$. In corollary \ref{CGSLS:cor:parSetUp3} we have a new setting for $\{\beta_k\}, \{\gamma_k\}$ and $\{\eta_k\}$ that lead to our desired improvement.


\begin{corollary}\label{CGSLS:cor:parSetUp3}
Let
\begin{align*}
\b\k =L\k\g\k,\qquad \G\k= L\k\g\k^3,\qquad\text{and}\qquad  \eta\k = \frac{c L\k\g\k\dx}{k} 
\end{align*}
for constant $c > 0$  and $L_1=tM$, where $t\in(0,1)$.Then \eqref{Alg:CGSLS:minep} is satisfied when
\begin{align*}
k\ge \frac{17 D_{\mathcal{X}}} {\sqrt[6]{t}}\sqrt{\frac{(c+1)M}{\epsilon}}.
\end{align*}
\end{corollary}

\begin{proof}
Since $\G\k=L\k\g\k^3 = (1-\g\k)\g\km$ and $L_1\le L\k\le 2M$ we have
\begin{align*}
\frac{1}{\G\k}- \frac{1}{\G\km} = \frac{\g\k}{\G\k}.
\end{align*}
Then
\begin{align*}
\sqrt[3]{\frac{1}{\G\k}} - \sqrt[3]{\frac{1}{\G\km}} &= \frac{\frac{1}{\G\k}-\frac{1}{\G\km}}{\sqrt[3]{\frac{1}{\G\k^2}}+\sqrt[3]{\frac{1}{\G\k\G\km}}+\sqrt[3]{\frac{1}{\G\km^2}}}\\
&\ge \frac{\frac{\g\k}{\G\k}}{3\sqrt[3]{\frac{1}{\G\k^2}}}\\
&=\frac{\g\k}{3\sqrt[3]{\G\k}}\\
&\ge \frac{\g\k}{3\sqrt[3]{L\k\g\k^3}}\\
&\ge \frac{1}{3\sqrt[3]{2M}}
\end{align*}
Summing up both sides of above inequality we obtain
\begin{align*}
\frac{1}{\sqrt[3]{\G\k}} - \frac{1}{\sqrt[3]{\G_1}}\ge \frac{k-1}{3\sqrt[3]{2M}},
\end{align*}
which implies that
\begin{align}\label{CGSLS:thm:qubGam:leq}
\G\k \le \frac{54 M}{(k-1)^3}.
\end{align}
In addition, since $\G\k = L\k\g\k^3$ we have 
\begin{align*}
\frac{1}{L\k} = \frac{\g\k^3}{\G\k},
\end{align*}
 and since $L_1\le L\k\le 2M$ we have
 \begin{align*}
 \frac{1}{2M}\le \frac{1}{L\k}\le \frac{1}{L_1}.
 \end{align*}
 Combining these two inequalities give that
 \begin{align*}
 \frac{1}{\sqrt[3]{2M}}\le \frac{\g\k}{\sqrt[3]{\G\k}}\le \frac{1}{\sqrt[3]{L_1}}.
 \end{align*}
So,
\begin{align*}
\frac{1}{\sqrt[3]{\G\k}} - \frac{1}{\sqrt[3]{\G\km}} &= \frac{\frac{\g\k}{\G\k}}{\sqrt[3]{\frac{1}{\G\k^2}}+\sqrt[3]{\frac{1}{\G\k\G\km}}+\sqrt[3]{\frac{1}{\G\km^2}}}\\
&= \frac{\sqrt[3]{\frac{1}{\G\k^2}}\frac{\g\k}{\sqrt[3]{\G\k}}}{\sqrt[3]{\frac{1}{\G\k^2}}+\sqrt[3]{\frac{1}{\G\k\G\km}}+\sqrt[3]{\frac{1}{\G\km^2}}}\\
&\le \frac{\g\k}{\sqrt[3]{\G\k}}\\
&\le \frac{1}{\sqrt[3]{L_1}}.
\end{align*} 
We have $L_1 = \G_1$. Summing up above inequality we get
\begin{align*}
\frac{1}{\sqrt[3]{\G\k}}\le \frac{k-1}{\sqrt[3]{L_1}}+\frac{1}{\sqrt[3]{L_1}} = \frac{k}{\sqrt[3]{L_1}}
\end{align*}
Therefore,
\begin{align*}
\G\k\ge \frac{L_1}{k^3}
\end{align*}
or
\begin{align*}
L\k\g\k^3\ge\frac{L_1}{K^3}
\end{align*}
which implies that
\begin{align*}
\frac{1}{\g\k^3}\le\frac{L\k k^3}{L_1}
\end{align*}
or
\begin{align}\label{CGSLS:thm:qubGam:geq}
\frac{1}{\g\k}\le k\sqrt[3]{\frac{2M}{L_1}}.
\end{align}

Hence, using \eqref{CGSLS:thm:qubGam:leq}, \eqref{CGSLS:thm:qubGam:geq} and Theorem \ref{CGSLS:mainthm}  we have
\begin{align*}
f(y\k) - \ell\k(x) &\le \frac{\epsilon}{2} + \G\k\sum_{i=1}^{k}\frac{\g_i\beta_i}{2\G_i}\pr{\norm{x-x_{i-1}}^2 - \norm{x-x)i}^2}\\
&\qquad +\G\k\sum_{i=1}^{k}\frac{\g_i\eta_i}{\G_i} - \sum_{i=1}^{k}\frac{\g_i}{2\G_i}\pr{\beta_i-L_i\g_i}\norm{x_i-x_{i-1}}^2\\
&= \frac{\epsilon}{2} + \G\k\pr{\sum_{i=1}^{k}\frac{\g_i\beta_i}{2\G_i}\pr{\norm{x-x_{i-1}}^2 - \norm{x-x)i}^2} +\sum_{i=1}^{k}\frac{\g_i\eta_i}{\G_i}}\\
&\le \frac{\epsilon}{2} + \G\k\pr{\frac{\dx}{\g\k}+c\sum_{i=1}^{k}\frac{\dx}{i\g\i}}\\
&\le \frac{\epsilon}{2} + \dx \G\k\pr{\frac{1}{\g\k}+c\sum_{i=1}^{k}\sqrt[3]{\frac{2M}{L_1}}}\\
&= \frac{\epsilon}{2} + \dx\pr{\frac{\G\k}{\g\k}+ck\sqrt[3]{\frac{2M}{L_1}}\G\k}\\
&\le \frac{\epsilon}{2} + \dx\pr{\frac{54M}{(k-1)^3} k\sqrt[3]{\frac{2M}{L_1}}+ck\sqrt[3]{\frac{2M}{L_1}}\frac{54M}{(k-1)^3}}\\
&= \frac{\epsilon}{2} + \dx\frac{(c+1)108Mk\sqrt[3]{\frac{2M}{L_1}}}{(k-1)^3}
\end{align*}

So, to have
\begin{align}\label{CGSLS:thm:k:epsilon/2}
\frac{(c+1)108\dx Mk\sqrt[3]{\frac{2M}{L_1}}}{(k-1)^3} \le \frac{\epsilon}{2}
\end{align}
we need
\begin{align*}
\frac{1}{k^2}\le \frac{k}{(k-1)^3}\le \frac{\epsilon}{2}\frac{\sqrt[3]{\frac{L_1}{2M}}}{108\dx M}=\frac{\epsilon\sqrt[3]{L_1}}{(c+1)216\dx \sqrt[3]{2M^4}}
\end{align*}
or
\begin{align}\label{CGSLS:thm:k:epsilon/2:2}
k\ge \sqrt{\frac{(c+1)216 \dx\sqrt[3]{2M^4}}{\epsilon\sqrt[3]{L_1}}} = \frac{D_X\sqrt{216\sqrt[3]{2}}\sqrt[3]{M^2}\sqrt{c+1}}{\sqrt{\epsilon}\sqrt[6]{L_1}}.
\end{align}
Therefore, if $L_1 = cM$ for some $c\in(0,1)$ and
\begin{align*}
k\ge \frac{17 D_{\mathcal{X}}} {\sqrt[6]{c}}\sqrt{\frac{(c+1)M}{\epsilon}}.
\end{align*}
then \eqref{CGSLS:thm:k:epsilon/2:2} and therefore \eqref{CGSLS:thm:k:epsilon/2} will also hold.
\end{proof}

Note that even when $L_1$ is significantly smaller than the true Lipschitz constant $M$, in order to get an epsilon solution, the increase in number of iterations is not significant. For example, for $t=0.01$ the number of outer iterations is approximately bounded by
\begin{align*}
17\sqrt{c+1} D_{\mathcal{X}}\sqrt{\frac{5M}{\epsilon}}.
\end{align*}


We finish this chapter by mentioning the fact that the constant $c$ in Corollary \ref{CGSLS:cor:parSetUp3} needs to be tuned for best practical performance.

